Scalable Deductive Verification of Data-Level Parallel Programs

This paper introduces several techniques that improve the scalability of the deductive verification of data-level programs working on arrays and matrices. First of all, we introduce a technique to rewrite expressions with (nested) quantifiers, so suitable triggers can be generated for these expressions. We have proven this rewrite technique correct in a theorem prover. Second, we make reasoning about potentially overlapping arrays easier, by providing specification constructs to indicate and verify that two arrays are not aliases, or that they are immutable, so they can be modelled as mathematical sequences. All our techniques are implemented in the VerCors program verifier. We illustrate how our techniques improve scalability through a large number of experiments. Using our techniques on a set of typical GPU kernels, we achieve a reduction of verification time by, on average, a factor of 9, with outliers being up to 150 times faster. Additionally, applying these techniques to earlier experiments and an earlier case study of a radio telescope pipeline permitted the verification of results which were previously unobtainable and significantly reduced the verification time.

==> prelude.tex <==
%!TEX root = main.tex



\newenvironment{proofsketch}{\paragraph{Proof sketch.}}{\\}

\makeatletter
% Taken from: https://tex.stackexchange.com/a/69076/5764
% \zsaveposx is defined since 2011/12/05 v2.23 of zref-savepos
\@ifundefined{zsaveposx}{\let\zsaveposx\zsavepos}{}
\makeatother
\newcounter{hposcnt}
\renewcommand*{\thehposcnt}{hpos\number\value{hposcnt}}
\newcommand*{\SP}{% set position
  \stepcounter{hposcnt}%
  \zsaveposx{\thehposcnt s}%
}
\makeatletter
\newcommand*{\UP}{% use previous position
  \zsaveposx{\thehposcnt u}%
  \zref@refused{\thehposcnt s}%
  \zref@refused{\thehposcnt u}%
  \kern\zposx{\thehposcnt s}sp\relax
  \kern-\zposx{\thehposcnt u}sp\relax
}
\makeatother

% Command for PVL text in math mode
\newcommand{\pvm}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\gtid}{\ensuremath{\backslash\pvm{gtid}}}

% \DeclareNewFootnote{default}
\RequirePackage{tikz}
\usetikzlibrary{automata,positioning,decorations.pathreplacing,calc,arrows}

\definecolor{clr-background}{RGB}{255,255,255}
\definecolor{clr-background-pvl}{RGB}{245,245,245}
\definecolor{clr-text}{RGB}{0,0,0}
\definecolor{clr-string}{RGB}{0, 128, 0}
\definecolor{clr-variable}{RGB}{0,0,0}
%\definecolor{clr-comment}{RGB}{64, 128, 128}
\definecolor{clr-comment}{rgb}{0.30, 0.50, 0.80}
\definecolor{clr-preprocessor}{RGB}{128,128,128}
%\definecolor{clr-keyword}{RGB}{0, 128, 0}
\definecolor{clr-keyword}{rgb}{0.5, 0.0, 0.13}
%\definecolor{clr-type}{RGB}{0, 0, 255}
\definecolor{clr-type}{rgb}{0.5, 0.0, 0.13}
\definecolor{clr-class}{RGB}{0, 0, 255}
%\definecolor{clr-operator}{RGB}{64,64,64}
\definecolor{clr-operator}{rgb}{0.10, 0.30, 0.60}
\definecolor{clr-number}{RGB}{0,0,0}
%\definecolor{clr-constant}{RGB}{136, 0, 0}
\definecolor{clr-constant}{rgb}{0.10, 0.30, 0.60}
\definecolor{ao}{rgb}{0.0, 0.3, 0.0}
\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\definecolor{ceruleanblue}{rgb}{0.30, 0.50, 0.80}
\definecolor{darkblue}{rgb}{0,0,0.40}

\newcommand{\halide}{\textsc{Halide}\xspace}
\newcommand{\haliver}{\textsc{HaliVer}\xspace}
\newcommand{\vercors}{\textsc{VerCors}\xspace}
\newcommand{\coq}{Coq\xspace}
\newcommand{\pvl}{\textsc{Pvl}\xspace}
\newcommand{\cogent}{\textsc{Cogent}\xspace}
\newcommand{\isabellehol}{\textsc{Isabelle/HOL}\xspace}
\newcommand{\compcert}{\textsc{CompCert}\xspace}
\newcommand{\alpinist}{\textsc{Alpinist}\xspace}
\newcommand{\opencl}{\textsc{OpenCL}\xspace}
\newcommand{\cuda}{\textsc{CUDA}\xspace}
\newcommand{\java}{\textsc{Java}\xspace}
\newcommand{\viper}{\textsc{Viper}\xspace}
\newcommand{\openmp}{\textsc{OpenMP}\xspace}
\def\CC{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\tiny\bf ++}}\xspace}
\def\C{\textsc{C}\xspace}
\newcommand{\lean}{\textsc{Lean}\xspace}

\newcommand{\OpenCL}{\textsc{OpenCL}\xspace}

%\RequirePackage{multirow}


%\RequirePackage{paralist}
%\RequirePackage{float}
%\newfloat{lstfloat}{htbp}{lop}
%\floatname{lstfloat}{Listing}
%\def\lstfloatautorefname{Listing} % needed for hyperref/auroref
\newcommand*{\ditto}{\textquotedbl}

\lstdefinestyle{unique}{
  breaklines,
  escapeinside={@}{@},
  basicstyle=\ttfamily\color{clr-text}\lst@ifdisplaystyle\scriptsize\fi,
  literate=%
    {=>>}{{{\color{clr-operator}$\mapsto$\lst@whitespacefalse}}}1
    {->}{{{\color{clr-operator}$\rightarrow$\lst@whitespacefalse}}}1
    {_1}{{{$_{1}$\lst@whitespacefalse}}}1
	{_2}{{{$_{2}$\lst@whitespacefalse}}}1,
  morekeywords={Float, Int, Bool, Rational, Void, Unique, Pointer, Struct, ADT, Set, Tuple},
  keywordstyle=\color{burgundy},
  commentstyle=\color{clr-comment},
  morecomment=[l][\it\color{clr-comment}]{//},
  % morecomment=[l][]{\\},
  xleftmargin=0.05\textwidth,
  xrightmargin=0.01\textwidth,
  classoffset=3,
  %Types
  morekeywords={case, of, map},
  keywordstyle=\color{burgundy},
}
\def\unInl{\lstinline[style=unique, breaklines]}

\lstdefinestyle{halide}{
	breaklines,
	language=C++,
	backgroundcolor=\color{clr-background},
	basicstyle=\ttfamily\color{clr-text}\lst@ifdisplaystyle\scriptsize\fi,
	stringstyle=\color{clr-string},
	identifierstyle=\color{clr-variable},
	commentstyle=\color{clr-comment},
	directivestyle=\color{clr-preprocessor},
	keywordstyle=\bf\color{clr-keyword},
	numbers=left,
	tabsize=2,
	columns=fullflexible,
	alsoletter=\,*,
	frame = single,
	framesep=\fboxsep,
	framerule=\fboxrule,
	mathescape=true,
	showstringspaces=false,
	showspaces=false,
	xleftmargin=0.05\textwidth,
	xrightmargin=0.01\textwidth,
	morekeywords={inline},
	classoffset=0,
	morekeywords={par, barrier},
	classoffset=1,
	mathescape,
	%Halide classes
	morekeywords={ImageParam,OutputImageParam,Param,,Annotation,Func,Var,Expr,RVar,where,RDom,Buffer, pipeline, fun, allocate, label, rdom, select, produce, store, split, compute_at, compute_inline, compute_root, store_at, store_root, unroll, parallel, serial, fuse, reorder, clone_in, unrolled, consume, vectorize, gpu, compute_with, update, atomic, specialize, gpu_tile, TailStrategy, GuardWithIf, RoundUp, ShiftInwards, gpu_blocks, gpu_threads, for},
	keywordstyle=\color{clr-class},
  	% Special characters
    literate=%
	    {0}{{{0\lst@whitespacefalse}}}1
	    {1}{{{1\lst@whitespacefalse}}}1
	    {2}{{{2\lst@whitespacefalse}}}1
	    {3}{{{3\lst@whitespacefalse}}}1
	    {4}{{{4\lst@whitespacefalse}}}1
	    {5}{{{5\lst@whitespacefalse}}}1
	    {6}{{{6\lst@whitespacefalse}}}1
	    {7}{{{7\lst@whitespacefalse}}}1
	    {8}{{{8\lst@whitespacefalse}}}1
	    {9}{{{9\lst@whitespacefalse}}}1
	    {\\}{{{\color{clr-constant}$\backslash$\lst@whitespacefalse}}}1
	    {\\forall}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
	    {\\forall*}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
	    {\\exists}{{{\color{clr-operator}$\exists$\lst@whitespacefalse}}}1
	    {\\gtid}{{{\color{ceruleanblue}$\backslash$gtid\lst@whitespacefalse}}}4
	    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
	    {<=}{{{\color{clr-operator}$\leq$\lst@whitespacefalse}}}1
	    {==}{{{\color{clr-operator}$\equiv$\lst@whitespacefalse}}}1
	    {\*\*}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
	    {\&\&}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    	{||}{{{\color{clr-operator}$\vee$\lst@whitespacefalse}}}1
        % {>}{{{\color{clr-operator}$>$\lst@whitespacefalse}}}1
        {>=}{{{\color{clr-operator}$\geq$\lst@whitespacefalse}}}1
        {==>}{{{\color{clr-operator}$\Rightarrow$\lst@whitespacefalse}}}1
        {=>>}{{{\color{clr-operator}$\mapsto$\lst@whitespacefalse}}}1
        {!=}{{{\color{clr-operator}$\neq$\lst@whitespacefalse}}}1
        {uint16_t}{{{\color{clr-type}uint16\_t\lst@whitespacefalse}}}8
        {__m128}{{{\color{clr-type}\_\_m128\lst@whitespacefalse}}}6
        {__m128i}{{{\color{clr-type}\_\_m128i\lst@whitespacefalse}}}7
        {int*}{{{{\color{clr-type}int}*\lst@whitespacefalse}}}4
        {float*}{{{{\color{clr-type}float}*\lst@whitespacefalse}}}4
        {\\result}{{{\color{clr-constant}$\backslash$result\lst@whitespacefalse}}}6
        {\\in}{{{\color{clr-constant}$\backslash$in\lst@whitespacefalse}}}3
        {\{:}{{{\color{clr-constant}\{:\lst@whitespacefalse}}}2
        {:\}}{{{\color{clr-constant}:\}\lst@whitespacefalse}}}2
        {\\pow}{{{\color{clr-constant}$\backslash$pow\lst@whitespacefalse}}}4
        %{\\old}{{{\color{darkblue}$\backslash$old\lst@whitespacefalse}}}4
        {~}{{{\ }}}1,    
    classoffset=3,
	%Types
	morekeywords={forall,trigger,requires, dim,extent,stride,min,ensures, loop_invariant, loop, invariant, invariant_perm, let, context, context_perm, context_everywhere, write, read, pipeline_requires, pipeline_ensures, assert, assume, fold,unfold, unfolding, decreases, ghost, pure, opaque, reveal, inhale, exhale, given, yields,
	unique, immutable, unique_field, unique_pointer_field, pointer_length, pointer_block_length, pointer_block_offset, perm, adt, polarity_dependent, ltid},
	keywordstyle=\color{clr-constant},
	emph={int4, int, long, short, char, double, float, unsigned, void, bool, bool1, uint16, m128i, Array, seq, resource, for, const, par, struct},
	emphstyle=\color{clr-type},
	morekeywords=[1]{Perm},
	classoffset=0,
	keywordstyle=\color{darkblue},
	morecomment=[l][\color{clr-keyword}\bf]{\#pragma},
	morecomment=[is][]{[/*@}{@*/},
	morecomment=[l][\color{clr-comment}]{//@},
	moredelim=*[il][]{//~},
	%moredelim=*[il][]{//@},
	escapeinside={|}{|},
}

% black version of halide
\lstdefinestyle{halideb}{
	breaklines,
	language=C++,
	backgroundcolor=\color{clr-background},
	basicstyle=\ttfamily\color{clr-text}\lst@ifdisplaystyle\scriptsize\fi,
	stringstyle=\color{clr-text},
	identifierstyle=\color{clr-text},
	commentstyle=\color{clr-text},
	directivestyle=\color{clr-text},
	keywordstyle=\bf\color{clr-text},
	numbers=left,
	tabsize=2,
	columns=fullflexible,
	alsoletter=\,*,
	frame = single,
	framesep=\fboxsep,
	framerule=\fboxrule,
	mathescape=true,
	showstringspaces=false,
	showspaces=false,
	xleftmargin=0.05\textwidth,
	xrightmargin=0.01\textwidth,
	morekeywords={inline},
	classoffset=0,
	morekeywords={par, barrier},
	classoffset=1,
	mathescape,
	%Halide classes
	morekeywords={ImageParam,OutputImageParam,Param,,Annotation,Func,Var,Expr,RVar,where,RDom,Buffer, pipeline, fun, allocate, label, rdom, select, produce, store, split, compute_at, compute_inline, compute_root, store_at, store_root, unroll, parallel, serial, fuse, reorder, clone_in, unrolled, consume, vectorize, gpu, compute_with, update, atomic, specialize, gpu_tile, TailStrategy, GuardWithIf, RoundUp, ShiftInwards, gpu_blocks, gpu_threads, for},
	keywordstyle=\color{clr-text},
  	% Special characters
    literate=%
	    {0}{{{0\lst@whitespacefalse}}}1
	    {1}{{{1\lst@whitespacefalse}}}1
	    {2}{{{2\lst@whitespacefalse}}}1
	    {3}{{{3\lst@whitespacefalse}}}1
	    {4}{{{4\lst@whitespacefalse}}}1
	    {5}{{{5\lst@whitespacefalse}}}1
	    {6}{{{6\lst@whitespacefalse}}}1
	    {7}{{{7\lst@whitespacefalse}}}1
	    {8}{{{8\lst@whitespacefalse}}}1
	    {9}{{{9\lst@whitespacefalse}}}1
	    {\\}{{{\color{clr-text}$\backslash$\lst@whitespacefalse}}}1
	    {\\forall}{{{\color{clr-text}$\forall$\lst@whitespacefalse}}}1
	    {\\forall*}{{{\color{clr-text}$\forall$\lst@whitespacefalse}}}1
	    {\\exists}{{{\color{clr-text}$\exists$\lst@whitespacefalse}}}1
	    {\\gtid}{{{\color{clr-text}$\backslash$gtid\lst@whitespacefalse}}}4
	    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
	    {<=}{{{\color{clr-text}$\leq$\lst@whitespacefalse}}}1
	    {==}{{{\color{clr-text}$\equiv$\lst@whitespacefalse}}}1
	    {\*\*}{{{\color{clr-text}$\wedge$\lst@whitespacefalse}}}1
	    {\&\&}{{{\color{clr-text}$\wedge$\lst@whitespacefalse}}}1
    	{||}{{{\color{clr-text}$\vee$\lst@whitespacefalse}}}1
        % {>}{{{\color{clr-operator}$>$\lst@whitespacefalse}}}1
        {>=}{{{\color{clr-text}$\geq$\lst@whitespacefalse}}}1
        {==>}{{{\color{clr-text}$\Rightarrow$\lst@whitespacefalse}}}1
        {=>>}{{{\color{clr-text}$\mapsto$\lst@whitespacefalse}}}1
        {!=}{{{\color{clr-text}$\neq$\lst@whitespacefalse}}}1
        {uint16_t}{{{\color{clr-text}uint16\_t\lst@whitespacefalse}}}8
        {__m128}{{{\color{clr-text}\_\_m128\lst@whitespacefalse}}}6
        {__m128i}{{{\color{clr-text}\_\_m128i\lst@whitespacefalse}}}7
        {int*}{{{{\color{clr-text}int}*\lst@whitespacefalse}}}4
        {\\result}{{{\color{clr-text}$\backslash$result\lst@whitespacefalse}}}6
        {\\in}{{{\color{clr-text}$\backslash$in\lst@whitespacefalse}}}3
        {\{:}{{{\color{clr-text}\{:\lst@whitespacefalse}}}2
        {:\}}{{{\color{clr-text}:\}\lst@whitespacefalse}}}2
        {\\pow}{{{\color{clr-text}$\backslash$pow\lst@whitespacefalse}}}4
        %{\\old}{{{\color{clr-text}$\backslash$old\lst@whitespacefalse}}}4
        {~}{{{\ }}}1,    
    classoffset=3,
	%Types
	morekeywords={forall,trigger,requires, dim,extent,stride,min,ensures, loop_invariant, loop, invariant, invariant_perm, let, context, context_perm, context_everywhere, write, read, pipeline_requires, pipeline_ensures, assert, assume, fold,unfold, unfolding, decreases, ghost, pure, opaque, reveal, inhale, exhale, given, yields,
	unique, immutable, unique_field, unique_pointer_field,Perm, pointer_length, pointer_block_length, pointer_block_offset, perm, adt, polarity_dependent, ltid},
	keywordstyle=\color{clr-text},
	emph={int4, int, long, short, char, double, float, unsigned, void, bool, bool1, uint16, m128i, Array, seq, resource, for, const, par},
	emphstyle=\color{clr-text},    
	classoffset=0,
	keywordstyle=\bf\color{clr-text},
	morecomment=[l][\color{clr-text}\bf]{\#pragma},
	morecomment=[is][]{[/*@}{@*/},
	morecomment=[l][\color{clr-text}]{//@},
	moredelim=*[il][]{//~},
	%moredelim=*[il][]{//@},
	escapeinside={|}{|},
}

\lstdefinestyle{halide2}{
style = halide,
%Remove all literals
literate=%
	    {0}{{{0\lst@whitespacefalse}}}1
	    {1}{{{1\lst@whitespacefalse}}}1
	    {2}{{{2\lst@whitespacefalse}}}1
	    {3}{{{3\lst@whitespacefalse}}}1
	    {4}{{{4\lst@whitespacefalse}}}1
	    {5}{{{5\lst@whitespacefalse}}}1
	    {6}{{{6\lst@whitespacefalse}}}1
	    {7}{{{7\lst@whitespacefalse}}}1
	    {8}{{{8\lst@whitespacefalse}}}1
	    {9}{{{9\lst@whitespacefalse}}}1
	    {\\}{{{\color{clr-constant}$\backslash$\lst@whitespacefalse}}}1
	    {\\forall}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
	    {\\forall*}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
	    {\\exists}{{{\color{clr-operator}$\exists$\lst@whitespacefalse}}}1
	    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
	    {<=}{{{\color{clr-operator}$\leq$\lst@whitespacefalse}}}1
	    {==}{{{\color{clr-operator}$\equiv$\lst@whitespacefalse}}}1
%	    {\*\*}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
	    {\&\&}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    	{||}{{{\color{clr-operator}$\vee$\lst@whitespacefalse}}}1
        % {>}{{{\color{clr-operator}$>$\lst@whitespacefalse}}}1
        {>=}{{{\color{clr-operator}$\geq$\lst@whitespacefalse}}}1
        {==>}{{{\color{clr-operator}$\Rightarrow$\lst@whitespacefalse}}}1
        {=>>}{{{\color{clr-operator}$\mapsto$\lst@whitespacefalse}}}1
        {!=}{{{\color{clr-operator}$\neq$\lst@whitespacefalse}}}1
        {uint16_t}{{{\color{clr-type}uint16\_t\lst@whitespacefalse}}}8
        {__m128}{{{\color{clr-type}\_\_m128\lst@whitespacefalse}}}6
        {__m128i}{{{\color{clr-type}\_\_m128i\lst@whitespacefalse}}}7
        {int*}{{{{\color{clr-type}int}*\lst@whitespacefalse}}}4
        {float*}{{{{\color{clr-type}float}*\lst@whitespacefalse}}}4
        {\\result}{{{\color{clr-constant}$\backslash$result\lst@whitespacefalse}}}6
        {\\in}{{{\color{clr-constant}$\backslash$in\lst@whitespacefalse}}}3
        {\{:}{{{\color{clr-constant}\{:\lst@whitespacefalse}}}2
        {:\}}{{{\color{clr-constant}:\}\lst@whitespacefalse}}}2
        {\\pow}{{{\color{clr-constant}$\backslash$pow\lst@whitespacefalse}}}4
        %{\\old}{{{\color{clr-constant}$\backslash$old\lst@whitespacefalse}}}4
        {__global__}{{{\color{clr-type}\_\_global\_\_\lst@whitespacefalse}}}9
        {~}{{{\ }}}1,
}

\lstdefinestyle{pvlin}{
style = halide,
autogobble=true,
commentstyle=\color{ceruleanblue},
emphstyle=\color{clr-type},
}

% black version of pvlin
\lstdefinestyle{pvlinb}{
style = halideb,
autogobble=true,
commentstyle=\color{ceruleanblue},
emphstyle=\color{clr-type},
}

\lstdefinestyle{pvl}{
 style=pvlin,
 numbers=left,
 backgroundcolor=\color{clr-background-pvl},
 classoffset=5,
}

% black version of pvl
\lstdefinestyle{pvlb}{
 style=pvlinb,
 numbers=left,
 backgroundcolor=\color{clr-background-pvl},
 classoffset=5,
}

\lstdefinestyle{annC}{
style=pvl,
moredelim=*[s][]{/*@}{@*/},
moredelim=*[l][]{//@},
}

\lstdefinestyle{pvlNoLabel}{
 style = pvl,
 escapeinside={^}{^},
 morecomment=*[is][]{|}{|},
}

\lstdefinestyle{pvl2}{
style=pvl,
backgroundcolor=\color{clr-background-pvl},
keywordstyle = [2]{\color{lime}},
otherkeywords={Perm,write,context,requires,ensures,loop_invariant},
morekeywords=[2]{;},
%escapeinside={@}{@},
classoffset=3,
%Numbers
literate=%
	{_0}{{{$_{0}$\lst@whitespacefalse}}}1
	{_1}{{{$_{1}$\lst@whitespacefalse}}}1
	{_2}{{{$_{2}$\lst@whitespacefalse}}}1
	{_3}{{{$_{3}$\lst@whitespacefalse}}}1
	{_4}{{{$_{4}$\lst@whitespacefalse}}}1
	{_5}{{{$_{5}$\lst@whitespacefalse}}}1
	{_6}{{{$_{6}$\lst@whitespacefalse}}}1
	{_7}{{{$_{7}$\lst@whitespacefalse}}}1
	{_8}{{{$_{8}$\lst@whitespacefalse}}}1
	{_9}{{{$_{9}$\lst@whitespacefalse}}}1
	%{_k}{{{$_{k}$\lst@whitespacefalse}}}1
	{_\{k-1\}}{{{$_{k-1}$\lst@whitespacefalse}}}3
	{_\{i-1\}}{{{$_{i-1}$\lst@whitespacefalse}}}3
	{_\{i+1\}}{{{$_{i+1}$\lst@whitespacefalse}}}3
	{loop_invariant}{{{\color{darkblue}{loop\_invariant}\lst@whitespacefalse}}}9
        {old}{{{\color{darkblue}old\lst@whitespacefalse}}}9
        {gtid}{{{\color{darkblue}gtid\lst@whitespacefalse}}}9
	%{_i}{{{$_{i}$\lst@whitespacefalse}}}1
	{^\{-1\}}{{{$^{-1}$\lst@whitespacefalse}}}1
    {\#-}{{{\color{clr-comment}<}}}1
    {-\#}{{{\color{clr-comment}>}}}1
    {\\}{{{\color{clr-constant}$\backslash$\lst@whitespacefalse}}}1
    {\\forall}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
    {\\forall*}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
    {\\exists}{{{\color{clr-operator}$\exists$\lst@whitespacefalse}}}1
    %{\\gtid}{{{\color{ceruleanblue}$\backslash$gtid\lst@whitespacefalse}}}4
    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
    {<=}{{{\color{clr-operator}$\leq$\lst@whitespacefalse}}}1
    {==}{{{\color{clr-operator}$\equiv$\lst@whitespacefalse}}}1
    {\*\*}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    {\&\&}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    {||}{{{\color{clr-operator}$\vee$\lst@whitespacefalse}}}1
    {>}{{{\color{clr-operator}$>$\lst@whitespacefalse}}}1
    {>=}{{{\color{clr-operator}$\geq$\lst@whitespacefalse}}}1
    {==>}{{{\color{clr-operator}$\Rightarrow$\lst@whitespacefalse}}}1
    {=>>}{{{\color{clr-operator}$\mapsto$\lst@whitespacefalse}}}1
    {!=}{{{\color{clr-operator}$\neq$\lst@whitespacefalse}}}1
	%{_f}{{{$_{f}$\lst@whitespacefalse}}}1
    {\{:}{{{\color{clr-constant}\{:\lst@whitespacefalse}}}1
    {:\}}{{{\color{clr-constant}:\}\lst@whitespacefalse}}}1
   {int*}{{{{\color{clr-type}int}*\lst@whitespacefalse}}}4
   {float*}{{{{\color{clr-type}float}*\lst@whitespacefalse}}}4
    {~}{{{\ }}}1,
   %moredelim=*[is][]{\{:}{:\}},
}

\lstdefinestyle{pvl3}{
style=pvl,
backgroundcolor=\color{clr-background-pvl},
escapeinside={@}{@},
classoffset=3,
%Numbers
literate=%
	{_k}{{{$_{k}$\lst@whitespacefalse}}}1
	{_\{k-1\}}{{{$_{k-1}$\lst@whitespacefalse}}}3
	{_\{i-1\}}{{{$_{i-1}$\lst@whitespacefalse}}}3
	{_\{i+1\}}{{{$_{i+1}$\lst@whitespacefalse}}}3
	{loop_invariant}{{{\color{burgundy}{loop\_invariant}\lst@whitespacefalse}}}9
	{_i}{{{$_{i}$\lst@whitespacefalse}}}1
	{^\{-1\}}{{{$^{-1}$\lst@whitespacefalse}}}1
    {\\}{{{\color{clr-constant}$\backslash$\lst@whitespacefalse}}}1
    {\\forall}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
    {\\forall*}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
    {\\exists}{{{\color{clr-operator}$\exists$\lst@whitespacefalse}}}1
    {\\gtid}{{{\color{clr-constant}$\backslash$gtid\lst@whitespacefalse}}}4
    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
    {<=}{{{\color{clr-operator}$\leq$\lst@whitespacefalse}}}1
    {==}{{{\color{clr-operator}$\equiv$\lst@whitespacefalse}}}1
    {\*\*}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    {\&\&}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    {||}{{{\color{clr-operator}$\vee$\lst@whitespacefalse}}}1
    % {>}{{{\color{clr-operator}$>$\lst@whitespacefalse}}}1
    {>=}{{{\color{clr-operator}$\geq$\lst@whitespacefalse}}}1
    {==>}{{{\color{clr-operator}$\Rightarrow$\lst@whitespacefalse}}}1
    {=>>}{{{\color{clr-operator}$\mapsto$\lst@whitespacefalse}}}1
    {!=}{{{\color{clr-operator}$\neq$\lst@whitespacefalse}}}1
	{_f}{{{$_{f}$\lst@whitespacefalse}}}1
    {~}{{{\ }}}1
    {\{:}{{{\color{clr-constant}\{:\lst@whitespacefalse}}}2
    {:\}}{{{\color{clr-constant}:\}\lst@whitespacefalse}}}2,
}

\lstdefinestyle{pvl4}{
style=pvl2,
backgroundcolor=\color{clr-background-pvl},
%escapeinside={@}{@},
classoffset=3,
%Numbers
literate=%
	{_1}{{{$_{1}$\lst@whitespacefalse}}}1
	{_k}{{{$_{k}$\lst@whitespacefalse}}}1
	{_\{k-1\}}{{{$_{k-1}$\lst@whitespacefalse}}}3
    {\\forall}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
    {<=}{{{\color{clr-operator}$\leq$\lst@whitespacefalse}}}1
    {==}{{{\color{clr-operator}$\equiv$\lst@whitespacefalse}}}1
    {\&\&}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
}

\lstdefinestyle{pvlcomments}{
style=pvl,
backgroundcolor=\color{clr-background-pvl},
basicstyle=\ttfamily\color{clr-comment}\lst@ifdisplaystyle\scriptsize\fi,
stringstyle=\color{clr-comment},
identifierstyle=\color{clr-comment},
commentstyle=\color{clr-comment},
directivestyle=\color{clr-comment},
keywordstyle=\bf\color{clr-comment},
rulecolor=\color{black},
%escapeinside={@}{@},
classoffset=3,
%Numbers
literate=%
	{_0}{{{$_{0}$\lst@whitespacefalse}}}1
	{_1}{{{$_{1}$\lst@whitespacefalse}}}1
	{_2}{{{$_{2}$\lst@whitespacefalse}}}1
	{_3}{{{$_{3}$\lst@whitespacefalse}}}1
	{_4}{{{$_{4}$\lst@whitespacefalse}}}1
	{_5}{{{$_{5}$\lst@whitespacefalse}}}1
	{_6}{{{$_{6}$\lst@whitespacefalse}}}1
	{_7}{{{$_{7}$\lst@whitespacefalse}}}1
	{_8}{{{$_{8}$\lst@whitespacefalse}}}1
	{_9}{{{$_{9}$\lst@whitespacefalse}}}1
	{_k}{{{$_{k}$\lst@whitespacefalse}}}1
	{_\{k-1\}}{{{$_{k-1}$\lst@whitespacefalse}}}3
	{_\{i-1\}}{{{$_{i-1}$\lst@whitespacefalse}}}3
	{_\{i+1\}}{{{$_{i+1}$\lst@whitespacefalse}}}3
	{loop_invariant}{{{\color{clr-comment}{loop\_invariant}\lst@whitespacefalse}}}9
	%{_i}{{{$_{i}$\lst@whitespacefalse}}}1
	{^\{-1\}}{{{$^{-1}$\lst@whitespacefalse}}}1
    {\#}{{{\color{clr-comment}$\mid$\lst@whitespacefalse}}}1
    {\\}{{{\color{clr-comment}$\backslash$\lst@whitespacefalse}}}1
    {\\forall}{{{\color{clr-comment}$\forall$\lst@whitespacefalse}}}1
    {\\forall*}{{{\color{clr-comment}$\forall$\lst@whitespacefalse}}}1
    {\\exists}{{{\color{clr-comment}$\exists$\lst@whitespacefalse}}}1
    {\\gtid}{{{\color{darkblue}$\backslash$gtid\lst@whitespacefalse}}}4
    {\\old}{{{\color{darkblue}$\backslash$old\lst@whitespacefalse}}}4
    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
    {<=}{{{\color{clr-comment}$\leq$\lst@whitespacefalse}}}1
    {==}{{{\color{clr-comment}$\equiv$\lst@whitespacefalse}}}1
    {\*\*}{{{\color{clr-comment}$\wedge$\lst@whitespacefalse}}}1
    {\&\&}{{{\color{clr-comment}$\wedge$\lst@whitespacefalse}}}1
    {||}{{{\color{clr-comment}$\vee$\lst@whitespacefalse}}}1
    {>}{{{\color{clr-comment}$>$\lst@whitespacefalse}}}1
    {>=}{{{\color{clr-comment}$\geq$\lst@whitespacefalse}}}1
    {==>}{{{\color{clr-comment}$\Rightarrow$\lst@whitespacefalse}}}1
    {=>>}{{{\color{clr-comment}$\mapsto$\lst@whitespacefalse}}}1
    {!=}{{{\color{clr-comment}$\neq$\lst@whitespacefalse}}}1
	%{_f}{{{$_{f}$\lst@whitespacefalse}}}1
    {\{:}{{{\color{clr-comment}\{:\lst@whitespacefalse}}}1
    {:\}}{{{\color{clr-comment}:\}\lst@whitespacefalse}}}1
    {~}{{{\ }}}1,
	emph={int4, int, long, short, char, double, float, unsigned, void, bool, bool1, uint16, m128i, Array, seq, resource, for, const, par},
	emphstyle=\color{clr-comment},    
	classoffset=0,
    %moredelim=*[is][]{\{:}{:\}},
}

\lstdefinestyle{pvlblack}{
style=pvlb,
backgroundcolor=\color{clr-background-pvl},
basicstyle=\ttfamily\color{clr-text}\lst@ifdisplaystyle\scriptsize\fi,
stringstyle=\color{clr-text},
identifierstyle=\color{clr-text},
commentstyle=\color{clr-text},
directivestyle=\color{clr-text},
keywordstyle=\bf\color{clr-text},
rulecolor=\color{black},
%escapeinside={@}{@},
classoffset=3,
%Numbers
literate=%
	{_0}{{{$_{0}$\lst@whitespacefalse}}}1
	{_1}{{{$_{1}$\lst@whitespacefalse}}}1
	{_2}{{{$_{2}$\lst@whitespacefalse}}}1
	{_3}{{{$_{3}$\lst@whitespacefalse}}}1
	{_4}{{{$_{4}$\lst@whitespacefalse}}}1
	{_5}{{{$_{5}$\lst@whitespacefalse}}}1
	{_6}{{{$_{6}$\lst@whitespacefalse}}}1
	{_7}{{{$_{7}$\lst@whitespacefalse}}}1
	{_8}{{{$_{8}$\lst@whitespacefalse}}}1
	{_9}{{{$_{9}$\lst@whitespacefalse}}}1
	{_k}{{{$_{k}$\lst@whitespacefalse}}}1
	{_\{k-1\}}{{{$_{k-1}$\lst@whitespacefalse}}}3
	{_\{i-1\}}{{{$_{i-1}$\lst@whitespacefalse}}}3
	{_\{i+1\}}{{{$_{i+1}$\lst@whitespacefalse}}}3
	{loop_invariant}{{{\color{clr-text}{loop\_invariant}\lst@whitespacefalse}}}9
	%{_i}{{{$_{i}$\lst@whitespacefalse}}}1
	{^\{-1\}}{{{$^{-1}$\lst@whitespacefalse}}}1
    {\\}{{{\color{clr-text}$\backslash$\lst@whitespacefalse}}}1
    {\\forall}{{{\color{clr-text}$\forall$\lst@whitespacefalse}}}1
    {\\forall*}{{{\color{clr-text}$\forall$\lst@whitespacefalse}}}1
    {\\exists}{{{\color{clr-text}$\exists$\lst@whitespacefalse}}}1
    {\\gtid}{{{\color{clr-text}$\backslash$gtid\lst@whitespacefalse}}}4
    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
    {\#-}{{{\color{clr-text}<}}}1
    {-\#}{{{\color{clr-text}>}}}1
    {<}{{{\color{clr-text}$<$\lst@whitespacefalse}}}1
    {<=}{{{\color{clr-text}$\leq$\lst@whitespacefalse}}}1
    {==}{{{\color{clr-text}$\equiv$\lst@whitespacefalse}}}1
    {\*\*}{{{\color{clr-text}$\wedge$\lst@whitespacefalse}}}1
    {\&\&}{{{\color{clr-text}$\wedge$\lst@whitespacefalse}}}1
    {||}{{{\color{clr-text}$\vee$\lst@whitespacefalse}}}1
    {>}{{{\color{clr-text}$>$\lst@whitespacefalse}}}1
    {>=}{{{\color{clr-text}$\geq$\lst@whitespacefalse}}}1
    {==>}{{{\color{clr-text}$\Rightarrow$\lst@whitespacefalse}}}1
    {=>>}{{{\color{clr-text}$\mapsto$\lst@whitespacefalse}}}1
    {!=}{{{\color{clr-text}$\neq$\lst@whitespacefalse}}}1
	%{_f}{{{$_{f}$\lst@whitespacefalse}}}1
    {\{:}{{{\color{clr-text}\{:\lst@whitespacefalse}}}1
    {:\}}{{{\color{clr-text}:\}\lst@whitespacefalse}}}1
    {~}{{{\ }}}1,
	emph={int4, int, long, short, char, double, float, unsigned, void, bool, bool1, uint16, m128i, Array, seq, resource, for, const, par},
	emphstyle=\color{clr-text},    
	classoffset=0,
    %moredelim=*[is][]{\{:}{:\}},
}

\def\pvlinlinetwo{\lstinline[style=pvl2, breaklines]}
\def\pvlinlinefour{\lstinline[style=pvl4, breaklines]}
\def\pvlinlinec{\lstinline[style=pvlcomments, breaklines]}
\def\pvlinlineb{\lstinline[style=pvlblack, breaklines]}

%\newcommand{\pvlinlinecomment}[1]{{\color{clr-comment}{\pvlinlinefour|#1|}}}

\lstdefinestyle{struc}{
language = C++,
commentstyle=\color{ceruleanblue},
columns=fullflexible,
%framexleftmargin=1mm,
xleftmargin=1mm,
alsoletter=\,*,
morekeywords={def, in, foreach},
morekeywords={pure, invariant, ensures, requires, context, decreases, context_everywhere, \length, par, \result,
  \forall, \forall*, **, Perm,send,receive,loop_invariant,for, Barrier, barrier, resource, CLK_GLOBAL_MEM_FENCE, get_global_id, seq, frac, inline, tail, head, none, }, %barrier
breaklines=true,
tabsize=2,%\fontsize{6}{10}\selectfont\color{ao}\tt,%\footnotesize\color{ao}\tt,
keywordstyle=\color{burgundy}\tt,
mathescape=true,
showstringspaces=false,
basicstyle=\ttfamily,
showspaces=false,
emph={ddecal, assign_solutions},
emphstyle=\color{clr-type},
%escapechar={\#},
xleftmargin=0.05\textwidth,
xrightmargin=0.01\textwidth,
literate=%
    {0}{{{0\lst@whitespacefalse}}}1
    {1}{{{1\lst@whitespacefalse}}}1
    {2}{{{2\lst@whitespacefalse}}}1
    {3}{{{3\lst@whitespacefalse}}}1
    {4}{{{4\lst@whitespacefalse}}}1
    {5}{{{5\lst@whitespacefalse}}}1
    {6}{{{6\lst@whitespacefalse}}}1
    {7}{{{7\lst@whitespacefalse}}}1
    {8}{{{8\lst@whitespacefalse}}}1
    {9}{{{9\lst@whitespacefalse}}}1
    {\\forall}{{{\color{clr-operator}$\forall$\lst@whitespacefalse}}}1
    % {<}{{{\color{clr-operator}$<$\lst@whitespacefalse}}}1
    {<=}{{{\color{clr-operator}$\leq$\lst@whitespacefalse}}}1
    {==}{{{\color{clr-operator}$ \equiv $\lst@whitespacefalse}}}1
    %{==}{{{\color{clr-operator}$ == $\lst@whitespacefalse}}}1
    {\&\&}{{{\color{clr-operator}$\wedge$\lst@whitespacefalse}}}1
    {||}{{{\color{clr-operator}$\vee$\lst@whitespacefalse}}}1
    % {>}{{{\color{clr-operator}$>$\lst@whitespacefalse}}}1
    {>=}{{{\color{clr-operator}$\geq$\lst@whitespacefalse}}}1
    {==>}{{{\color{clr-operator}$\Rightarrow$\lst@whitespacefalse}}}1
    {=>>}{{{\color{clr-operator}$\mapsto$\lst@whitespacefalse}}}1
    {_v,d}{{{\color{clr-operator}$_{v,d}$\lst@whitespacefalse}}}1
    {_v}{{{\color{clr-operator}$_{\texttt{v}}$\lst@whitespacefalse}}}1
    {_dd}{{{\color{clr-operator}$_{\texttt{d}}$\lst@whitespacefalse}}}1
    {_00}{{{\color{clr-operator}$_{00}$\lst@whitespacefalse}}}1
    {_11}{{{\color{clr-operator}$_{11}$\lst@whitespacefalse}}}1
    {^H}{{{\color{clr-operator}$^{H}$\lst@whitespacefalse}}}1
    {!=}{{{\color{clr-operator}$\neq$\lst@whitespacefalse}}}1,
    float=t,
    numbers=left,
    frame = single,
    framesep=\fboxsep,
    framerule=\fboxrule,
    backgroundcolor=\color{clr-background-pvl},
    basicstyle=\ttfamily\lst@ifdisplaystyle\scriptsize\fi,
    emph={[2]subtract_direction, add, add_direction, solve_direction, step},
    emphstyle={[2]\color{clr-type}\underbar},
}

\def\halinline{\lstinline[style=halide, breaklines]}
\def\pvlinline{\lstinline[style=pvl, breaklines]}
\def\pvli{\lstinline[style=pvl, breaklines]}


\newcommand{\hoare}[1]{\big\{ #1 \big\}}
%\newcommand{\env}[1]{\{ #1 \}}
%\newcommand{\toE}[1]{\mathbb{E} \llbracket #1 \rrbracket}
%\newcommand{\toT}[1]{\mathbb{T} \llbracket #1 \rrbracket}
%\newcommand{\redlabel}[1]{{}^{\textcolor{blue}{(#1)}}}
\newcommand{\mt}[1]{\textbf{\texttt{#1}}}
%\newcommand{\divE}[1]{\ensuremath{1}}%\/}}%/_{E}}}
%\newcommand{\modE}[1]{\ensuremath{}\mod_{E}}
\newcommand{\divE}{\ensuremath{/_E}~}
\newcommand{\modE}{\ensuremath{~\text{mod}_E}~}


% VerCors things
\newcommand*{\predicate}[1][predicate]{\hyperlink{predicate}{#1}\xspace}
\newcommand*{\fold}[1][fold]{\hyperlink{fold}{#1}\xspace}
\newcommand*{\lemmaver}[1][lemma]{\hyperlink{lemmaver}{#1}\xspace}
\newcommand*{\pure}[1][pure]{\hyperlink{pure}{#1}\xspace}
\newcommand*{\quantifier}[1][quantifier]{\hyperlink{quantifier}{#1}\xspace}
\newcommand*{\nonlinear}[1][nonlinear]{\hyperlink{nonlinear}{#1}\xspace}
\newcommand*{\adt}[1][adt]{\hyperlink{adt}{#1}\xspace}
\newcommand*{\ghost}[1][ghost]{\hyperlink{ghost}{#1}\xspace}
\newcommand*{\given}[1][given]{\hyperlink{given}{#1}\xspace}
\newcommand*{\trigger}[1][trigger]{\hyperlink{trigger}{#1}\xspace}
\newcommand*{\sequence}[1][sequence]{\hyperlink{sequence}{#1}\xspace}
\newcommand*{\parblock}[1][parallel block]{\hyperlink{parblock}{#1}\xspace}
\newcommand*{\gpukernelver}[1][GPU kernel]{\hyperlink{gpukernel}{#1}\xspace}
\newcommand*{\contract}[1][contract]{\hyperlink{contract}{#1}\xspace}
\newcommand*{\permission}[1][permission]{\hyperlink{permission}{#1}\xspace}
\newcommand*{\decrease}[1][decrease]{\hyperlink{decrease}{#1}\xspace}
\newcommand*{\inhale}[1][inhale]{\hyperlink{inhale}{#1}\xspace}


% Halide things
\newcommand*{\produce}[1][produce]{\hyperlink{produce}{#1}\xspace}
\newcommand*{\consume}[1][consume]{\hyperlink{produce}{#1}\xspace}
\newcommand*{\tuple}[1][tuple]{\hyperlink{tuple}{#1}\xspace}
\newcommand*{\select}[1][select]{\hyperlink{tuple}{#1}\xspace}
\newcommand*{\reduction}[1][reduction]{\hyperlink{reduction}{#1}\xspace}
\newcommand*{\buffer}[1][buffer]{\hyperlink{buffer}{#1}\xspace}

\newcommand*{\pipeline}[1][pipeline]{\hyperlink{pipeline}{#1}\xspace}
\newcommand*{\haldefinition}[1][definition]{\hyperlink{halide-definition}{#1}\xspace}
\newcommand*{\halparallel}[1][parallel]{\hyperlink{loop-parallel}{#1}\xspace}
\newcommand*{\vectorize}[1][vectorize]{\hyperlink{loop-parallel}{#1}\xspace}
\newcommand*{\halsplit}[1][split]{\hyperlink{loop-alter}{#1}\xspace}
\newcommand*{\reorder}[1][reorder]{\hyperlink{loop-alter}{#1}\xspace}
\newcommand*{\fuse}[1][fuse]{\hyperlink{loop-alter}{#1}\xspace}
\newcommand*{\computeat}[1][compute at]{\hyperlink{func-order}{#1}\xspace}
\newcommand*{\storeat}[1][store at]{\hyperlink{func-order}{#1}\xspace}
\newcommand*{\func}[1][func]{\hyperlink{func}{#1}\xspace}
\newcommand*{\storagefolding}[1][func]{\hyperlink{func-order}{#1}\xspace}


% GPU things
\newcommand*{\synchronisation}[1][synchronisation]{\hyperlink{synchronisation}{#1}\xspace}
\newcommand*{\instructionlevel}[1][instruction-level]{\hyperlink{instruction-level}{#1}\xspace}
\newcommand*{\datarace}[1][data race]{\hyperlink{data-race}{#1}\xspace}
\newcommand*{\barrier}[1][barrier divergence]{\hyperlink{synchronisation}{#1}\xspace}
\newcommand*{\barrierdivergence}[1][barrier divergence]{\hyperlink{synchronisation}{#1}\xspace}
\newcommand*{\finesynchronisation}[1][fine-grained synchronisation]{\hyperlink{synchronisation}{#1}\xspace}
\newcommand*{\dynamicparallelism}[1][dynamic parallelism]{\hyperlink{dynamic-parallelism}{#1}\xspace}
\newcommand*{\warpprimitive}[1][warp primitive]{\hyperlink{dynamic-parallelism}{#1}\xspace}
\newcommand*{\threaddivergence}[1][thread divergence]{\hyperlink{thread-divergence}{#1}\xspace}
\newcommand*{\sharedmemory}[1][shared memory]{\hyperlink{gpu-memory}{#1}\xspace}
\newcommand*{\coalesced}[1][coalesced]{\hyperlink{gpu-memory}{#1}\xspace}
\newcommand*{\gpukernel}[1][GPU kernel]{\hyperlink{gpukernelver}{#1}\xspace}

\newcommand*{\memorylocality}[1][memory locality]{\hyperlink{memory-locality}{#1}\xspace}

\newcommand*{\openmpback}[1][\openmp]{\hyperlink{openmp}{#1}\xspace}

\usetikzlibrary{tikzmark}
% Command to place a TikZ anchor at the current position
\newcommand{\tmark}[1]{%
  \tikz[overlay,remember picture,baseline] \coordinate (#1) at (0,0) {};}
\newcommand{\hl}[3]{%
  \draw[#1,line width=14pt,opacity=0.3]%
    ([yshift=4pt]#2) -- ([yshift=4pt]#3);%
}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

==> results/blas_level1.tex <==
\newcommand{\widthPadre}{0.9}
\subfloat[\label{tab:blaslevel1}\texttt{CLBLAS level 1 kernels}]{
\resizebox{\widthPadre\textwidth}{!}{
\begin{tabular}{l|lll|l|rrr|rrr r|rrr r|rrr r|rrr rr}
\hline
 & & & & & \multicolumn{3}{c|}{\textbf{Base}}& \multicolumn{4}{c}{\textbf{Unique}}& \multicolumn{4}{c}{\textbf{Immutable}}& \multicolumn{4}{c}{\textbf{Extract}}& \multicolumn{4}{c}{\textbf{All}}\\
\textbf{Kernel} & $\#_{imm}$ & $\#_{p}$ & $\#_{A}$ & \textbf{Result} & \textbf{\#} & \textbf{T} & $\mathbf{\sigma}$ & \textbf{\#} & \textbf{T} & $\mathbf{\sigma}$ & \textbf{Speedup} & \textbf{\#} & \textbf{T} & $\mathbf{\sigma}$ & \textbf{Speedup} & \textbf{\#} & \textbf{T} & $\mathbf{\sigma}$ & \textbf{Speedup} & \textbf{\#} & \textbf{T} & $\mathbf{\sigma}$ & \textbf{Speedup}\\
\hline
xamax &  1 &  4 &  31 & \checkmark&  10 & 34 & 1&  10&  30 & 1& 1.1&  10&  29 & 1& 1.2&  10& \cellcolor{ForestGreen!25} 24 & 1& 1.4&  10& \cellcolor{ForestGreen!25} 24 & 2& 1.4 \\
\hline
xasum &  1 &  2 &  37 & \checkmark&  10 & 20 & 1&  10&  19 & 2& 1.1&  10&  16 & 1& 1.2&  10& \cellcolor{ForestGreen!25} 13 & 1& 1.5&  10& \cellcolor{ForestGreen!25} 13 & 1& 1.5 \\
\hline
xaxpy$^\dagger$ &  1 &  1 &  16 & \checkmark&  9 & 66 & 47&  10&  19 & 6& 3.3&  10&  24 & 7& 2.6&  9&  13 & 2& 4.8&  10& \cellcolor{ForestGreen!25} 9 & 1& 6.9 \\
\hline
 & & && $\times$& 1 & 23 & -& 0 &  &  && 0 &  &  && 1 & 13 & - && 0 &  &  & \\
\hline
xcopy$^\dagger$ &  1 &  1 &  15 & \checkmark&  8 & 52 & 15&  10&  16 & 5& 6.3&  10&  15 & 4& 6.7&  10&  22 & 7& 4.6&  10& \cellcolor{ForestGreen!25} 10 & 1& 10.1 \\
\hline
 & & && $\times$& 2 & 296 & 18& 0 &  &  && 0 &  &  && 0 &  &  && 0 &  &  & \\
\hline
xdot &  2 &  2 &  24 & \checkmark&  10 & 20 & 1&  10&  18 & 1& 1.1&  10&  16 & 1& 1.2&  10&  15 & 1& 1.3&  10& \cellcolor{ForestGreen!25} 12 & 1& 1.7 \\
\hline
xhad$^\dagger$ &  2 &  1 &  19 & \checkmark&  8 & 450 & 149&  10&  73 & 23& 8.0&  10&  48 & 14& 12.1&  10&  54 & 14& 10.8&  10& \cellcolor{ForestGreen!25} 12 & 1& 48.4 \\
\hline
 & & && $\times$& 2 & 1104 & 788& 0 &  &  && 0 &  &  && 0 &  &  && 0 &  &  & \\
\hline
xnrm2 &  1 &  2 &  54 & \checkmark&  10 & 21 & 1&  10&  20 & 1& 1.1&  10&  18 & 1& 1.2&  10&  15 & 1& 1.4&  10& \cellcolor{ForestGreen!25} 14 & 1& 1.5 \\
\hline
xswap$^\dagger$ &  0 &  2 &  19 & \checkmark&  10 & 66 & 23&  10&  32 & 13& 2.1& - & - & - &&  10&  28 & 11& 2.4&  10& \cellcolor{ForestGreen!25} 12 & 1& 5.5 \\
\hline
xscal$^\dagger$ &  0 &  1 &  13 & \checkmark&  10 & 8 & 1& - & - & - && - & - & - &&  10& \cellcolor{ForestGreen!25}\cellcolor{BrickRed!25} 10 & 2& 0.8& - & - & - & \\
\hline
\hline
Total & & & & & & 913 & 197 & & 463 & 28 & 2.0 & & 466 & 54 & 1.8 & & 388 & 19 & 2.4 & & 219 & 3 & 4.1  \\
\hline
\end{tabular}
}
}
\\

==> results/blas_level2.tex <==
\subfloat[\label{tab:blaslevel2}\texttt{CLBLAS level 2 kernels}]{
\resizebox{\widthPadre\textwidth}{!}{
\begin{tabular}{l|lll|l|rr|rr S[table-format=-4.1]|rr S[table-format=-4.1]|rr S[table-format=-4.1]|rr S[table-format=-4.1]r}
\hline
 & & & & & \multicolumn{2}{c|}{\textbf{Base}}& \multicolumn{3}{c}{\textbf{Unique}}& \multicolumn{3}{c}{\textbf{Immutable}}& \multicolumn{3}{c}{\textbf{Extract}}& \multicolumn{3}{c}{\textbf{All}}\\
\textbf{Kernel} & $\#_{cp}$ & $\#_{p}$ & $\#_{A}$ & \textbf{Result} & \textbf{\#} & \textbf{T} & \textbf{\#} & \textbf{T} & \textbf{Speedup} & \textbf{\#} & \textbf{T} & \textbf{Speedup} & \textbf{\#} & \textbf{T} & \textbf{Speedup} & \textbf{\#} & \textbf{T} & \textbf{Speedup}\\
\hline
xger$^\dagger$ &  2 &  3 &  69 & \checkmark& \cellcolor{BrickRed!25} 0 & & \cellcolor{ForestGreen!25} 9&  369& 5.3& \cellcolor{ForestGreen!25} 5&  981& 2.4& \cellcolor{ForestGreen!25} 3&  1443& 1.7& \cellcolor{ForestGreen!25} 10& \cellcolor{ForestGreen!25} 14& 151.5 \\
\hline
 & & && $\times$& 8 & 1751& 1 & 701 && 5 & 803 && 7 & 1149 && 0 &  & \\
\hline
 & & && T.O.& 2 & -& 0 &  && 0 &  && 0 &  && 0 &  & \\
\hline
xher$^\dagger$ &  1 &  3 &  37 & \checkmark&  3 & 1507&  10&  261& 3.0&  9&  280& 2.6&  5&  401& 2.2&  10& \cellcolor{ForestGreen!25} 42& 18.5 \\
\hline
 & & && $\times$& 7 & 465& 0 &  && 1 & 495 && 5 & 315 && 0 &  & \\
\hline
xher2$^\dagger$ &  2 &  5 &  56 & \checkmark& \cellcolor{BrickRed!25} 0 & & \cellcolor{ForestGreen!25} 2&  922& 0.7& \cellcolor{ForestGreen!25} 4&  731& 1.4& \cellcolor{BrickRed!25} 0&  & 1.4& \cellcolor{ForestGreen!25} 10& \cellcolor{ForestGreen!25} 48& 21.5 \\
\hline
 & & && $\times$& 10 & 1030& 8 & 1638 && 6 & 739 && 10 & 733 && 0 &  & \\
\hline
xtrsv$^\dagger$ &  2 &  3 &  68 & \checkmark&  8 & 1381&  10& \cellcolor{ForestGreen!25} 330& 5.5&  10&  610& 3.0&  9&  1217& 1.4&  10&  455& 4.0 \\
\hline
 & & && $\times$& 0 & & 0 &  && 0 &  && 1 & 1933 && 0 &  & \\
\hline
 & & && T.O.& 2 & -& 0 &  && 0 &  && 0 &  && 0 &  & \\
\hline
xgemv &  2 &  3 &  80 & \checkmark&  6 & 1664&  10&  380& 4.6&  10&  159& 11.1&  9&  787& 2.1&  10& \cellcolor{ForestGreen!25} 135& 13.0 \\
\hline
 & & && $\times$& 4 & 1905& 0 &  && 0 &  && 1 & 1411 && 0 &  & \\
\hline
\hline
Total & & & & & & 7514 & & 2867 & 2.6 & & 2699 & 2.8 & & 4466 & 1.7 & & 694 & 10.8  \\
\hline
\end{tabular}
}
}
\\
